Weak MSO: Automata and Expressiveness Modulo Bisimilarity

We prove that the bisimulation-invariant fragment of weak monadic second-order logic (WMSO) is equivalent to the fragment of the modal $\mu$-calculus where the application of the least fixpoint operator $\mu p.\varphi$ is restricted to formulas $\varphi$ that are continuous in $p$. Our proof is automata-theoretic in nature; in particular, we introduce a class of automata characterizing the expressive power of WMSO over tree models of arbitrary branching degree. The transition map of these automata is defined in terms of a logic $\mathrm{FOE}_1^\infty$ that is the extension of first-order logic with a generalized quantifier $\exists^\infty$, where $\exists^\infty x. \phi$ means that there are infinitely many objects satisfying $\phi$. An important part of our work consists of a model-theoretic analysis of $\mathrm{FOE}_1^\infty$.

==> automata-defs.tex <==
% !TEX root = main-wmso.tex


%%
\subsection{Automata over transition systems}
%\fcwarning{Check if this is the best way to present this.}
\fznote{I rewrote this informal introduction to parity automata. The original one is commented.}
In this section we provide an automata characterization of $\wmso$. To this aim, we first recall parity automata. Informally, those are automata working on transition systems, where each state $a \in A$ is assigned a natural number called parity (or priority). A (possibly infinite) run on input $\model$ is given at each step by the automaton observing a point $s\in |\model|$ in some state $a$. The transition map associates $s$ and $a$ with a formula $\Delta(a,\V(s))$ of a one-step language $\llang_1(A)$. Intuitively, $\Delta(a,\V(s))$ expresses constraints on the successors of $s$, from which depend the next state and point of $\model$ occurring in the run. The acceptance of $\model$ is determined by the priorities of the states encountered during the run.

\begin{comment}
In this article we will work with parity automata; they consist of a set $A$ of states which have an assigned parity (or priority) and a transition map which gives, for each state, a formula of a one-step language $\llang_1(A)$. Intuitively, the transition map denotes a set of possible `next states' on the automata together with constraints on the children of $s$. %Such constraints are defined using a one-step language $\llang_1(A)$.
%
These automata run on trees, at each step of a run the automaton is in a state $a\in A$ and is looking at a point $s\in |\model|$.
Runs can be infinite and the priorities of the states that are visited in the run are used to accept or reject the transition system.
\end{comment}

\begin{definition}\label{def:parity_aut}
An \emph{$\llang_1$-parity automaton} on alphabet $C$ is a tuple $\aut = \tup{A,\tmap,\pmap,a_I}$ s.t.
\begin{enumerate}[(i)]
\itemsep 0 pt
\item $A$ is a finite set of states of the automaton,
\item $a_I \in A$ is the initial state,
\item $\tmap: A\times C \to \llang^+_1(A)$ is the transition map,
\item $\pmap: A \to \nat$ is the parity map.
\end{enumerate}
\end{definition}

Given an arbitrary one-step language $\llang_1$, by $\yvAut(\llang_1)$ we denote the class of $\llang_1$-parity automata.

Let $\aut$ be an arbitrary $\llang_1$-parity automaton, for some one-step language $\llang_1$, and let $a, b \in A$. We say that $b$ is $\tmap$-reachable from $a$, if there is a sequence $a_0, \dots, a_k$ of states such that $a_0=a$, $a_k=b$ and for every $i<k$, there is $c_i \in C$ such that $a_{i+1}$ occurs in $\tmap(a_i,c_i)$.  The quasi-ordering $\ord$ on $A$ induced by the transition map $\tmap$ is defined by stating that $a \ord b$ if $b$ is $\tmap$-reachable from $a$.








\begin{definition}
Given a transition system $\model=\tup{T,R,V,s_I}$, the \emph{acceptance game}
$\mathcal{A}(\aut,\model)$ of $\aut$ on $\model$ is the parity game
defined according to the rules of the following table.
%
% \begin{table*}[ht]
%   \centering
\begin{center}
\fcwarning{Markings vs valuations...}\begin{tabular}{|l|c|l|c|}
 \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Position & Player & Admissible moves & Parity\\
  \hline
  $(a,s) \in A \times T$ & $\exists$ & $\{m : A \rightarrow \wp(R[s]) \mid (R[s],m) \models \tmap (a, V^\flat(s)) \}$ & $\pmap(a)$\\
  $m : A \rightarrow \wp(T)$ & $\forall$ & $\{(b,t) \mid t \in m(b)\}$ & $\max(\pmap[A])$\\
  \hline
 \end{tabular}
\end{center}
%  \caption{Acceptance game for parity automata}
%   \label{exists_asymmetric_game}
% \end{table*}
%
Finite matches of $\mathcal{A}(\aut,\model)$ are lost by the player
who gets stuck.
An infinite match of $\mathcal{A}(\aut,\model)$ is won by $\exists$ if
and only if the \emph{minimum} parity occurring infinitely often is even.
%
A transition system $\model$ is \emph{accepted} by $\aut$ if and only if $\exists$ has
a winning strategy in $\mathcal{A}(\aut,\model)@(a_I,s_I)$.
The collection of transition systems accepted by $\aut$, also called its \emph{language}, is denoted by
$\lng(\aut)$. The \emph{tree language} $\trees(\aut)$ accepted by $\aut$ is the collection of trees in $\lng(\aut)$.
%\fcwarning{We want (here) to define something more general than tree language (i.e. language)}
\end{definition}

\begin{lemma}
  \fcnote{Fabio, Yde, maybe this is a good place to put this.} If $\llang$ is closed under boolean duals then the class of $\llang$-parity automata is closed under complementation.
  \fznote{I think the statement should also assume: ``and if the class of $\llang$-parity automata is closed under the $(-)^{\star}$ transformation" (see Yde's mail), as this is a non completely trivial observation for $\wmso$-automata.}
\end{lemma}

\begin{fact}
  Anecdotic fact about (FOE/MSO)-parity automata corresponding to MSO on trees? or maybe should appear later.
\end{fact}
\begin{comment}
\begin{fact}[\cite{Walukiewicz96}] \label{t:msoauto}
For every \mso formula $\varphi$ there is an effectively constructible \foe_1-parity automaton $\aut_{\varphi}$ such that, for any tree $\model$, $$\model \in \trees(\aut_{\varphi}) \text{ iff } \model \models \aut_{\varphi}.$$
\end{fact}
\end{comment}


Given a one-step language $\llang_1$, a $\llang_1$-parity automaton on alphabet $C$ is called a \emph{weak} $\llang_1$-parity automaton if the following condition holds:
\begin{description}
\item[weakness:]  if  $a \ord b$ then $\pmap(a) \leq \pmap(b)$,
\end{description}

\begin{remark}
Any weak parity automaton $\aut$ is equivalent to a weak parity automaton $\aut'$ with $\pmap: A' \to \{0,1\}$. From now on we therefore consider only weak parity automata with priorities $0$ and $1$.
\end{remark}

%\fzwarning{I would not put this paragraph here, as the goal of characterizing WMSO on trees is still not explicit and then the story continues at a different level of abstraction with the definition of continuity. Moreover, I don't see the relation between AFMC and WMSO, for which the reader may think what you are conjecturing.}One could naively think that just adding the weakness condition to  $\yvAut(\foe_1)$ would be enough to capture \wmso (on trees), as by adding the weakness condition to $\yvAut(\fo_1)$-automata we can capture exactly the expressive power of the alternation free fragment. As remarked in \cite{Zanasi:Thesis:2012,DBLP:conf/lics/FacchiniVZ13} this is not true.
%In order to achieve this aim, we therefore have to add an additional restriction on the transition function.

\afwarning{Add something that explain why we have to add continuity condition?}

Let $\llang_1$ be a one-step language.
Recall from Section \ref{subsec:one-stepcont} the definition of a formula $\varphi \in \llang_1(A)$ being (co-)continuous in some $a \in A$.
Given a weak $\llang_1$-parity automaton on alphabet $C$, the continuity condition is defined as follows:
\begin{description}
\item[continuity:] let $a,b$ be states such that both $a\ord b$ and $b \ord a$ , and $c\in C$. If ${\pmap(b)}=1$  then $\tmap(b,c)$ is continuous in $a$. In case $\pmap(b)=0$, then $\tmap(b,c)$ is co-continuous in $a$.
\end{description}

Given an arbitrary one-step language $\llang_1$, by $\yvwAut(\llang_1)$ we denote the class of weak $\llang_1$-parity automata with the continuity condition.






%\begin{definition}%[Automata]
%The class of \emph{\wmso-automaton} is the class
%is a tuple $\aut = \tup{A,\tmap,\pmap,\ord}$ such that
%\begin{enumerate}[(i)]
%\itemsep 0 pt
%\item $A$ is a finite set of states of the automaton, %and $A_0, A_1$ is a partition of $A$
%\item $\ord$ is a quasi-ordering on $A$ (i.e., reflexive and transitive),
%\item $\tmap: A\times C \to {\olque}^+(A)$ %{\sf d}{\owmsoe}^+(A,A_0, A_1)
%    \fzerror{The target should be $\SLatt({\olque}^+(A))$, where $\SLatt$ has to be defined somewhere}
%is the transition map s.t. $\tmap(a,c) \in {\olque}^+(\{b\in A \mid a \ord b\})$,
%\item $\pmap: A \to \{0,1\}$ is the parity map, satisfying the following two conditions:
%        \fzwarning{Perhaps it is worth remarking that any weak automaton can be thought as one with parities only $0$ and $1$.}
%\begin{description}
%\item[weakness:]  if  $a \ord b$ and $b \ord a$ then $\pmap(a) = \pmap(b)$,
%     \fzwarning{I think is more convenient to express weakness without using the ordering $\ord$}
%     %where $\ord $ is the quasi-ordering on $A$ induced by $\tmap$,
%%\item[continuity:] if $a \in A_0$ then  $\pmap(a)$ is even, while if $a \in A_1$ then  $\pmap(a)$ is odd.
%\item[continuity:] let $a,b$ be states belonging to the same $\ord$-cycle and $c\in C$. If ${\pmap(b) = 1}$ then $\tmap(b,c)$ is continuous in $a$. In case $\pmap(b) = 0$ then $\tmap(b,c)$ is co-continuous in $a$.
%    \fzwarning{Where is co-continuity defined? At the moment, continuity in $a$ is actually defined later (Simulation section)}
%\end{description}
%\end{enumerate}
%\end{definition}



==> contoweak.tex <==
% !TEX root = main-wmso.tex

In this section we verify that every  $\contAFMC$-formula is equivalent to a $\WMSO$-formula.
%
Firstly, let us define, for every first-order variable $x$, a translation $ST_x$ from $\contAFMC$-formulas into $\WMSO$-formulas with only $x$ free as follows:

\begin{itemize}
\itemsep 0 pt
\item $ST_x(p)=p(x)$
\item $ST_x(\varphi \land \psi)=ST_x(\varphi) \land ST_x(\psi)$,
\item $ST_x(\varphi \lor \psi)=ST_x(\varphi) \lor ST_x(\psi)$,
\item $ST_x(\lnot \varphi)= \lnot ST_x(\varphi)$,
\item $ST_x(\Diamond \varphi)=\exists y (R(x,y) \land ST_y(\varphi)$),
\item $ST_x(\mu p. \varphi)= \exists p ( p(x) \land \forall y ( p(y) \to ST_y(\varphi) ))$.
\end{itemize}
Note that in $ST_x(\mu p. \varphi)$, the predicate $p$ which occurs in $ST_y(\varphi) $ is bounded by the outermost second order existential quantifier.
%

Let $(-)_\bullet$ be simply $ST_x$, for a given first-order variable $x$. Then, we prove the following theorem.

\begin{theorem}\label{thm:contransweak}
For every LTS $\model = \tup{T,R,\tscolors,s_I}$, the following two conditions are equivalent:
%
\begin{enumerate}
\itemsep 0pt
\item $\model \mmodels \varphi$,
\item $\model[x \mapsto s_I] \models \varphi_\bullet$.
\end{enumerate}
%
\end{theorem}
\begin{proof}
The proof goes by induction on the complexity of $\varphi$, the only critical step being the least fixpoint operator one.
Let therefore consider $\mu p. \varphi$. Recall that we assume, without loss of generality, that bounded and free variables are distinct in $\mu p. \varphi$.
We first show that $(1)$ implies $(2)$. Since $\model \mmodels \varphi$, \'Eloise has a winning strategy $f$ in $\egame(\mu p.\varphi,\model)@(\mu p.\varphi,s_I)$.
Define $p^\model \subseteq T$ to be the set of nodes $s \in T$ such that there is a (partial) match $\pi'$ satisfying
%
\begin{enumerate}[(1)]
\itemsep 0pt
\item $\pi'$ is $f$-guided,
\item every position of $\pi'$ is of the form $(\gamma,m)$, with $p$ occurring in $\gamma$, and%\fcwarning{Define `active in'}
\item the last position of $\pi'$ is of the form $(\mu p. \varphi, s)$.
\end{enumerate}
%
The key observation is that since $f$ is a winning strategy, all $f$-guided matches are finite, and that because $p$ is existential in $\varphi$, \eloise is the only player who picks successors in $\pi'$. As a consequence of K\"onig's Lemma, $p^\model$ is finite.
%
Using the induction hypothesis, it is easy to check that $\model[x \mapsto s_I] \models \exists p ( p(x) \land \forall y ( p(y) \to ST_y(\varphi) ))$ with $p \mapsto p^\model$ as a witness.

For the other direction, the idea is the following. Because $\model[x \mapsto s_I] \models ST_x(\varphi)$,
there is a finite set $p^\model$ such that $\model[x \mapsto s_I, p \mapsto p^\model] \models p(x) \land \forall y ( p(y) \to ST_y(\varphi) )$. The winning strategy for \'Eloise  in $\egame(\mu p.\varphi,\model)@(\mu p.\varphi,s_I)$ is thus defined as the composition of all winning strategies in $\egame(\varphi,\model[p \mapsto p^\model])@(\varphi,s)$ for $s \in p^\model$.
\end{proof}

%As an immediate consequence of the  Theorems \ref{t:wmsobis} and \ref{thm:contransweak} we get
\noindent This concludes the proof of Theorem~\ref{t:m1}, and in particular of the fact that
$\contAFMC = \WMSO/{\bis}$.

==> simulationBackup.tex <==
% !TEX root = main-wmso.tex

In this section we show that any $\wmso$-automaton can be simulated by a `two-sorted' one, where one sort is given by the automaton that we want to simulate and the other by a variant of its powerset construction.

For defining the latter, we first need some preliminaries. As usual, we define a lifting from types on states to types on macro-states. The distinction between empty and non-empty subsets of $A$ is to make sure that empty types on states are lifted to empty types on macro-states.

\begin{definition} Let $A$ be a set of unary predicates. Given a set $\Sigma \subseteq A$, its \emph{lifting} is the subset $\Sigma^{\p}$ of $\p(A)$ given by $\{\{S\} \mid S \in \Sigma \wedge S \neq \emptyset\} \cup \{S \mid S \in \Sigma \wedge S = \emptyset\}$.
\end{definition}

The next step is to define a translation on the sentences associated with the transition function of the starting $\wmso$-automaton. The idea is that we want to work with sentences that can be made true by assigning macro-states to finitely many nodes in the model, and ordinary states to all the other nodes.

\begin{definition}\label{DEF_finitary_lifting}
Let $\varphi \in \olque(A)$ be a sentence of shape
%
\begin{eqnarray}%\label{EQ_disjBF}
\dbnfofoe{\overline{T}}{\Pi \cup \Sigma} \land
\bigwedge_{S\in\Sigma} \qu y.\tau_S(y) \land \dqu y.\bigvee_{S\in\Sigma} \tau_S(y) .
\end{eqnarray}
%
for some $\Pi,\Sigma \subseteq \wp A$ and $T_i \subseteq A$. We define the sentence $\varphi^{\f}$ as follows:
 $$
\dbnfofoe{\overline{T}^{\p}}{\Pi^{\p} \cup \Sigma^{\p} \cup \Sigma} \land
\bigwedge_{S\in\Sigma} \qu y.\tau_S(y) \land \dqu y.\bigvee_{S\in\Sigma} \tau_S(y) .
$$
Following the notation of Definition \ref{def:basicform_folque}, $\varphi$ and $\varphi^{\f}$ can be represented respectively as $\dbnfolque{\overline{T}}{\Pi}{\Sigma}$ and $\dbnfolque{\overline{T}^{\p}}{\Pi^{\p} \cup \Sigma^{\p}}{\Sigma}$.
\end{definition}

Our desiderata on the translation $(-)^{\f}$ concern the notions of \emph{continuity} and \emph{functionality}.
%Recall the notion of one step model $\osmodel = (D,\val)$ from Section \ref{subsec:normalforms}.
%We can extend the notion of continuity from formulae of the modal $\mu$-calculus to sentences in $\olque(A)$, in the expected way:
A sentence $\varphi \in \olque(A)$ is \emph{continuous in $a \in A$} if, whenever $\varphi$ is true in a one-step model $(D,\val \: A \to \p(D))$, then there is a restriction $\val'$ of $\val$ such that $\varphi$ is true in $(D,\val')$. Also we let ``continuous in a set $B \subseteq A$'' mean ``continuous in $b$, for each $b \in B$''.

We say that a formula $\varphi$ is \emph{functional in $B \subseteq A$} if, whenever it is true in a model $(D,\val)$, then there is a restriction $\val'$ of $\val$ such that $\varphi$ is true in $(D,\val')$ and, for each $d \in D$, if $d \in \val'(a)$ for some $a \in B$, then $d \not\in V'(b)$ for any $b \in B\setminus \{a\}$.

\begin{lemma}\label{LEM_cont}
Let $\varphi \in \olque(A)$ and $\varphi^{\f}\in \olque(A\cup \p(A))$ be given as in Definition \ref{DEF_finitary_lifting}. Then $\varphi^{\f}$ is continuous and functional in $\p(A)$.
 \end{lemma}

\begin{proof}
Suppose that $(D,\val \: (A \cup \p(A)) \to \p(D))$ is a model where $\varphi^{\f}$ is true. By a careful observation of the shape of $\varphi^{\f}$, we can infer the following information on $(D,\val)$:
\begin{itemize}
   \item as the existential part of $\dbnfofoe{\overline{T}^{\p}}{\Pi^{\p} \cup \Sigma^{\p} \cup \Sigma}$ is true, there is a set $D_t \subseteq D$ consisting of exactly one witness for each type in $\overline{T}^{\p}$;
   \item as the universal part of $\dbnfofoe{\overline{T}^{\p}}{\Pi^{\p} \cup \Sigma^{\p} \cup \Sigma}$ is true, there is a set $D_s \subseteq D\setminus D_t$ containing all the elements not in $D_t$ witnessing a type in $\Sigma$, and a set $D_p = D\setminus D_t \cup D_s$ of elements witnessing a type in $\Pi^{\p} \cup \Sigma^{\p}$;
   \item as the subformula
   $$\bigwedge_{S\in\Sigma} \qu y.\tau_S(y) \land \dqu y.\bigvee_{S\in\Sigma} \tau_S(y)$$ is true, the set $D \setminus D_s = D_t \cup D_p$ is finite and, if $\Sigma$ is non-empty, the set $D_s$ is infinite.
 \end{itemize}
Following the partition $D_t \cup D_p \cup D_s$, we can associate with each element of $D$ exactly one of the types in $\overline{T}^{\p} \cup \Pi^{\p} \cup \Sigma^{\p} \cup \Sigma$. This association induces a restriction $\val'$ of $\val$ such that $(\varphi)^{\f}$ is true in $(D,\val')$. By definition $\val'$ assigns unary predicates from $\p(A)$ only to elements in the finite set $D_t \cup D_p$, meaning that $\varphi^{\f}$ is continuous in $\p(A)$. Furthermore, $\val'$ assigns at most one unary predicate to each element of $D_t \cup D_p$, because $\overline{T}^{\p} \cup \Pi^{\p} \cup \Sigma^{\p}$ is defined as the lifting of $\overline{T} \cup \Pi \cup \Sigma$. It follows that $\varphi^{\f}$ is also functional in $\p(A)$.
\end{proof}

The next definition is standard in powerset constructions for tree automata, to have a well-behaved notion of trace.

\begin{definition}\label{DEF_delta star} Let $\mb{A} = \langle A,a_I,\Delta,\Omega\rangle$ be a $\wmso$-automaton. Fix $a \in A$ and $c \in C$. The sentence $\Delta^{\star}(a,c)$ is defined as
\begin{eqnarray*}
      % \nonumber to remove numbering (before each equation)
        \Delta^{\star}(a,c) &:=& \Delta(a,c)[(a,b)\setminus b\mid b \in A],
      \end{eqnarray*}
where $\Delta(a,c)[(a,b)\setminus b\mid b \in A]$ denotes the sentence in $\olque(A\times A)$ obtained by replacing each occurrence of an unary predicate $b \in A$ in $\Delta(a,c)$ with the unary predicate $(a,b) \in A \times A$.
\end{definition}

We now combine the previous definitions to characterize the transition function associated with the macro-states. We use the notation $\shA$ for the set $\p(A \times A)$.

\begin{definition}\label{PROP_DeltaPowerset}
Let $\mb{A} = \langle A,a_I,\Delta,\Omega\rangle$ be a $\wmso$-automaton. Let $c \in C$ be a label and $Q \in \shA$ a binary relation on $A$. By Theorem \ref{thm:bfolque} there is a sentence $\Psi_{Q,c} \in \olque(A\times A)$ in basic form such that
\begin{eqnarray*}
% \nonumber to remove numbering (before each equation)
  \bigwedge_{a \in \m{Ran}(Q)} \Delta^{\star}(a,c) &\equiv& \Psi_{Q,c}.
\end{eqnarray*}
By definition $\Psi_{Q,c}$ is of the form $\bigvee_{1\leq i\leq k}\varphi_i$. We put $\shDe(Q,c) := \bigvee_{1\leq i\leq k}\varphi_i^{\f}$, where the translation $(-)^{\f}$ is given as in definition \ref{DEF_finitary_lifting}. Observe that $\shDe(Q,c)$ is of type $\olque(A \cup \shA)$.
\end{definition}

We have now all the ingredients to define our two-sorted automaton.

\begin{definition}\label{def:finitaryconstruct}
Let $\mb{A} = \langle A,a_I,\Delta,\Omega\rangle$ be a {\wmso-automaton}. We define the \emph{finitary construct over $\mb{A}$} as the automaton $\mb{A}^{\f} = \langle A^{\f},a_I^{\f},\Delta^{\f},\Omega^{\f}\rangle$ given by
\begin{eqnarray*}
      % \nonumber to remove numbering (before each equation)
        A^{\f} &:=& A \cup \shA \\
        %\leq^{2S} &:=& \leq\ \cup\ (\shA \times A)\ \cup\ (\shA \times \shA)\\
        a_I^{\f} &:=& \{a_I,a_I\}\\
        \Delta^{\f}(a,c) &:=& \Delta(a,c)\\
        \Delta^{\f}(R,c) &:=& \shDe(R,c) \vee \bigwedge_{a \in \m{Ran}(R)} \Delta(a,c)\\
        \Omega^{\f}(a) &:=& \Omega(a)\\
        \Omega^{\f}(R) &:=& 1
      \end{eqnarray*}
\end{definition}

The underlying idea of Definition \ref{def:finitaryconstruct} is the same of the  \emph{two-sorted construction} \cite[Def. 3.7]{Zanasi:Thesis:2012} for weak $\mso$-automata, the difference being the definition of $\shDe$, which now has to take care of conditions concerning the cardinality of nodes witnessing some type.

The next proposition fixes the desired properties of the finitary construct. To this purpose, first recall that a strategy for $\exists$ in an acceptance game $\mathcal{A}(\aut,\model)$ is \emph{functional in a set $B$} of states if it assigns at most one state from $B$ to each node in $\mb{T}$, and it is \emph{finitary in $B$} if it assigns states from $B$ only to finitely many nodes of $\mb{T}$.

\begin{lemma}\label{PROP_facts_finConstr} Let $\mb{A}$ be a $\wmso$-automaton and $\mb{A}^{\f}$ its finitary construct over $\mb{A}$. The following holds:
\begin{enumerate}
  \item $\mb{A}^{\f}$ is a $\wmso$-automaton. \label{point:finConstrAut}
  \item For any tree $\mb{T}$, if $\exists$ has a winning strategy in the game $\mathcal{A}(\aut,\model)@(a_I^{\f},s_I)$, then it has a winning strategy in the same game which is both functional and finitary in $\shA$. \label{point:finConstrStrategy}
  \item $\mb{A} \equiv \mb{A}^{\f}$. \label{point:finConstrEquiv}
  \end{enumerate}
\end{lemma}
\begin{proof} %As observed above, the finitary construction resembles the two-sorted construction.
We address each point separately.
\begin{enumerate}
  \item We need to show that $\mb{A}^{\f}$ is weak and respects the continuity condition. Weakness follows by observing that:
            \begin{enumerate}[(A)]
        \item the initial state and all macro-states from $\shA$ have the same parity;
        \item whenever the automaton reaches a state $ a \in A^{\f} \setminus \shA = A$, a simulation of the $\wmso$-automaton $\mb{A}$ begins and we can assume that no more states from $\shA$ can be reached.
      \end{enumerate}
      For continuity, the key observation is that, by definition of $\Delta^{\f}$, a macro-state from $\shA$ and a state from $A$ will never be part of the same cycle. Thus it suffices to verify the following:
      \begin{enumerate}
        \item for any $c \in C$ and $a,b \in A$ belonging to the same cycle, the continuity condition holds; \label{point:contA}
        \item for any $c \in C$ and $R,Q \in \shA$ belonging to the same cycle, the continuity condition holds; \label{point:contAsharp}
      \end{enumerate}
     Point \eqref{point:contA} holds because $\aut$ is a $\wmso$-automaton. For point \eqref{point:contAsharp}, we know that $Q$ can only appear in the disjunct $\shDe(R,c) = \bigvee_{1\leq i\leq k}\varphi_i^{\f}$ of $\Delta^{\f}(R,c)$. By Lemma \ref{LEM_cont}, we know that each $\varphi_i^{\f}$ is continuous in $\shA$. Then in particular $\Delta^{\f}(R,c)$ is continuous in $Q$. As all macro-states from $\shA$ have parity $1$, point \eqref{point:contAsharp} follows.
  \item   
  \item The proof is entirely analogous to the one presented in \cite[Prop. 3.9]{Zanasi:Thesis:2012} for the two-sorted construction. For the direction from left to right, it is immediate by definition of $\mb{A}^{\f}$ that a winning strategy for $\exists$ in $\mathcal{A}(\aut,\model)@(a_I,s_I)$ is also winning for $\exists$ in $\mathcal{A}(\mb{A}^{\f},\model)@(a_I^{\f},s_I)$.

      For the direction from right to left, let $f$ be a winning strategy for $\exists$ in $\mathcal{A}(\mb{A}^{\f},\model)@(a_I^{\f},s_I)$. The idea is to define a strategy $f'$ for $\exists$ in stages, while playing a match $\pi'$ in $\mathcal{A}(\aut,\model)@(a_I,s_I)$. In parallel to $\pi'$, a shadow match $\pi$ in $\mathcal{A}(\mb{A}^{\f},\model)@(a_I^{\f},s_I)$ is maintained, where $\exists$ plays according to the strategy $f$. For each round $z_i$, we want to keep the following relation between the two matches:
\smallskip
\begin{center}
\fbox{\parbox{8cm}{
\begin{enumerate}
  \item either basic positions of the form $(Q,s) \in \shA \times T$ and $(a,s) \in A \times T$ occur respectively in $\pi$ and $\pi'$, with $a \in \m{Ran}(Q)$,
  \item or the same basic position of the form $(a,s) \in A \times T$ occurs in both matches.
\end{enumerate}
}}\hspace*{0.3cm}($\ddag$)
\end{center}
\smallskip
The key observation is that, because $f$ is winning, a basic position of the form $(Q,s) \in \shA \times T$ can occur only for finitely many initial rounds $z_0,\dots,z_n$ that are played in $\pi^{2S}$, whereas for all successive rounds $z_n,z_{n+1},\dots$ only basic positions of the form $(a,s) \in A \times T$ are encountered. Indeed, if this was not the case then either $\exists$ would get stuck or the minimum parity occurring infinitely often would be odd, since states from $\shA$ have parity $1$.

It follows that enforcing a relation between the two matches as in ($\ddag$) suffices to prove that the defined strategy $f'$ is winning for $\exists$ in $\pi'$. For this purpose, consider any round $z_i$ that is played in $\pi'$ and $\pi$, respectively with basic positions $(a,s) \in A \times T$ and $(q,s) \in A^{\f} \times T$. In order to define the suggestion of $f'$ in $\pi'$, we distinguish two cases.
\begin{enumerate}
  \item First suppose that $(q,s)$ is of the form $(Q,s) \in \shA\times T$. By inductive hypothesis we assume that $a$ is in $\m{Ran}(Q)$ - which is indeed the case at the initial round, where $R = \shai = \{a_I,a_I\}$. Let $m_{Q,s} :A^{\f} \rightarrow \p(\R{s})$ be the marking suggested by $f$, verifying the sentence $\Delta^{\f}(Q,\V(s))$. We distinguish two further cases, depending on which disjunct of $\Delta^{\f}(Q,\V(s))$ is made true by $m_{Q,s}$.
      \begin{enumerate}[label*=\roman*,ref=\roman*]
        \item If $(\R{s},m_{Q,s})\models \bigwedge_{b \in \m{Ran}(Q)} \Delta(b,\V(s))$, then we let $\exists$ pick the marking $m_{Q,s}$. \label{point:marking1}
        \item If $(\R{s},m_{Q,s})\models \shDe(Q,\V(s))$, we let $\exists$ pick a marking $m_{a,s}:A \rightarrow \p (\R{s})$ defined by putting
            \begin{align*}
            % \nonumber to remove numbering (before each equation)
               m_{a,s}(b)\ :=\ \bigcup_{b \in \m{Ran}(Q')} &\{t \in \R{s} \mid t \in m_{Q,s}(Q')\} \\
               \cup\ \ \ \ \ & \{t \in \R{s} \mid t \in m_{Q,s}(b)\} .
            \end{align*} \label{point:marking2}
      \end{enumerate}
      It can be readily checked that the suggested move is admissible for $\exists$ in $\pi$, i.e. it makes $\Delta(a,\V(s))$ true in $\R{s}$. For case \eqref{point:marking2}, one has to observe how $\shDe$ is defined in terms of $\Delta$. In particular, the nodes assigned to $b$ by $m_{Q,s}$ have to be assigned to $b$ also by $m_{a,s}$, as they may be necessary to fulfill the condition, expressed with $\qu$ and $\dqu$, that infinitely many nodes witness some type, or that finitely many nodes do not witness some type.
      
      In order to show that we can maintain the relation $(\ddag)$ for another round, observe that case \eqref{point:marking1} corresponds to $\mb{A}^{\f}$ starting the simulation of $\aut$: any next position $(b,t)\in A \times T$ picked by player $\forall$ in $\pi'$ is also available for $\forall$ in $\pi$, and we end up in case $(\ddag .2)$. If (b) is the case, by definition of $m_{a,s}$, given the choice $(b,t)$ of $\forall$, there is some $Q' \in \shA$ such that $b$ is in $\m{Ran}(Q')$ and $(Q',t)$ is an available choice for $\forall$ in the shadow match $\pi$. By letting $\pi$ advance at round $z_{i+1}$ with such move, we are able to maintain $(\ddag .1)$ also in $z_{i+1}$.
  \item In the remaining case, inductively we are given with the same basic position $(a,s) \in A\times T$ both in $\pi$ and in $\pi'$. The marking suggested by $f$ in $\pi$ verifies $\Delta^{\f}(a,s) = \Delta(a,s)$, so we let it be also the choice of $\exists$ in the match $\pi'$. It is immediate that any next move of $\forall$ in $\pi'$ can be mirrored by the same move in $\pi$, meaning that we are able to maintain the same position - whence the relation $(\ddag)$ - also in the next round.
\end{enumerate}
In both cases, the suggestion of strategy $f'$ was a legitimate move for $\exists$ maintaining the relation $(\ddag)$ between the two matches for any next round $z_{i+1}$. It follows that $f'$ is a winning strategy for $\exists$ in $\mc{G}$.
      
      \begin{comment} SHORTER ALTERNATIVE VERSION OF THE PROOF
      The idea is to define a strategy $f'$ for $\exists$ in stages, while playing a match $\pi'$ in $\mathcal{A}(\aut,\model)@(a_I,s_I)$. In parallel to $\pi'$, a shadow match $\pi$ in $\mathcal{A}(\mb{A}^{\f},\model)@(a_I^{\f},s_I)$ is maintained, where $\exists$ plays according to the strategy $f$. Since $f$ is winning and all macro-states from $\shA$ have an odd parity, in finitely many rounds the shadow match $\pi$ reaches a stage where $\mb{A}^{\f}$ enters a state from $A$ and ``behaves as'' $\aut$ for all successive rounds. Thus $\pi$ can be assumed to have the following structure:
       \begin{enumerate}[(I)]
         \item there is an $n$ such that, for each round $z_i$ in the initial segment $z_0,z_1,\dots,z_n$ of $\pi$, a position of the form $(R,s) \in \shA \times T$ is visited and the marking suggested by $f$ makes the disjunct $\shDe(R,\sigma_C(s))$ of $\Delta^{\f}(R,\sigma_C(s))$ true in $\sigma_R(s)$.
         \item At round $z_{n+1}$ a basic position of the form $(Q,t) \in \shA \times T$ is visited. The marking suggested by $f$ makes the disjunct $\bigwedge_{a \in \m{Ran}(R)} \Delta(a,\sigma_C(t))$ of $\Delta^{\f}(Q,\sigma_C(t))$ true in $\sigma_R(t)$. \label{point:initialsegm}
         \item For all the next rounds $z_{n+2},z_{n+3},\dots$ only positions of the form $(a,s) \in A \times T$ are visited.
       \end{enumerate}
       In each round of the initial segment $z_0,z_1,\dots,z_n$ we can maintain the condition that, if a position $(R,s)$ is visited in $\pi$, then at the same round a position $(a,s)$ with $a \in \m{Ran}(R)$ occurs in $\pi'$. This holds for the initial round $z_0$. For the next ones $z_1,\dots,z_n$, it can be enforced by defining $f'$ in terms of $f$ in the standard way shown, for instance, in the proof of \cite[Prop. 3.9]{Zanasi:Thesis:2012}.
       \fzwarning{More details to be provided}
       Once $\pi$ reaches round $z_n$, say with position $(Q,t)$, the marking suggested by $f$ makes $\bigwedge_{a \in \m{Ran}(R)} \Delta(a,\sigma_C(t))$ true in $\sigma_R(t)$ ({\it cf.} point \eqref{point:initialsegm}). By assumption, at round $z_n$, $\pi'$ visits a position $(b,t)$ with $b \in \m{Ran}(Q)$. Then in particular the marking suggested by $f$ makes $\Delta(b,\sigma_C(t))$ true, and we let it be the suggestion of $f'$ at that stage. By definition of $\Delta^{\f}$, from the next round onwards we can maintain the same basic positions in $\pi$ and $\pi'$, and let $f'$ just be defined as $f$. As $\exists$ wins $\pi$, it will also win the match $\pi'$, meaning that $f'$ is a winning strategy.
       \end{comment}
\end{enumerate}
\end{proof}

%Details on the proof have to be provided. The idea is that the first statement is true because $\mb{A}^{\f}$ is a weak automaton and its continuity property follows by the continuity of $\mb{A}$ and Lemma \ref{LEM_cont}. The argument showing the second statement should be analogous to the one relating weak $\m{MSO}$-automata and their two-sorted construct, see \cite[Prop. 3.9]{Zanasi:Thesis:2012}. The third statement should again follow by Lemma \ref{LEM_cont}.

\begin{remark} While the finitary construction is a variant of the two-sorted one, it is worth noticing that the latter would have not been suitable for our purposes. Indeed, suppose to define the two-sorted construct $\mb{A}^{2S}$ over a $\wmso$-automaton $\mb{A}$, analogously to the case of weak $\MSO$-automata. Then $\mb{A}^{2S}$ will generally \emph{not} be a $\wmso$-automaton. The problem is with the continuity condition: since all macro-states in $\mb{A}^{2S}$ have parity $1$, whenever two of them, say $R$ and $Q$, occur in the same loop, then the sentence $\Delta^{2S}(R,c)$ should be continuous in $Q$. But this is not necessarily the case, since the truth of $\Delta^{2S}(R,c)$ may depend upon the truth of a subformula of the form $\exists^{\infty}x.Q(x)$, requiring $Q$ to be interpreted over infinitely many nodes.

As a consequence, we cannot use the two-sorted construction to show that $\wmso$-automata are closed under noetherian projection \cite[Def. 3]{DBLP:conf/lics/FacchiniVZ13}. This observation is coherent with the fact that $\m{WFMSO}$ is \emph{not} a fragment of $\m{WMSO}$.\end{remark} 

==> yv-contoweak.tex <==
% !TEX root = main-wmso.tex

\newcommand{\CFq}{\mathit{CF}(q)}
\newcommand{\ST}[1]{\mathit{ST}_{#1}}

\begin{convention}
We assume familiarity with the syntax and (game) semantics of the modal 
$\mu$-calculus $\mu\ML$ and of weak monadic second-order logic (WMSO).

We will only interpret these languages on tree models $(\bbT,r)$, with $r$
being the root of the tree; for convenience we assume that $r$ is part of
the signature of WMSO.

We let $\sfor$ denote the subformula relation, and let $\Sfor{\al}$ denote
the set of subformulas of a formula $\al$.
The first-order standard translation (with free variable $x$) of a modal formula
$\psi$ is denoted as $\ST{x}(\psi)$.
\end{convention}

\begin{definition}
Given a proposition letter $q$, we define the set $\CFq$ by the following 
grammar:
\[
\alpha \isbnf q \divbnf \psi
   \divbnf \al \land \al \divbnf \al \lor \al \divbnf \dia\al,
\]
where $\psi$ denotes an arbitrary modal formula in which $q$ does not 
occur.
\end{definition}

It follows from results by Fontaine \& Venema that a modal formula is 
continuous in $q$ iff it is equivalent to a formula in the fragment $\CFq$.

\begin{theorem}
For any $\al \in \CFq$ that is guarded in $q$, the formula $\mu q. \al$ can
be expressed in WMSO.
\end{theorem}

From now on we fix a proposition letter $q$ and a formula $\al \in \CFq$
that is guarded in $q$.
In addition, we assume that $q$ does occur in $\al$.

\begin{definition}
Let $H$ denote the least subset of $\Sfor{\al}$
%set of subformulas of $\al$ 
such that $\al \in H$,
and if $q$ occurs in $\be \in H$, then all immediate subformulas of $\be$
also belong to $H$.
\end{definition}

It is not hard to show that $H \sse \CFq$.
More in particular, $H$ consists of those subformulas $\be$ of $\al$ 
such that either $q$ occurs in $\beta$, or $\al$ has a subformula of the form 
$\be\lor\be'$ or $\be\land\be'$ such that $q$ occurs in $\be'$ but not in 
$\be$.

As a consequence of the definition, any full match $\pi$ of an evaluation 
game $\EG(\al,\bbS)$ has an initial part $\pi'$ in which only formulas in 
$H$ are under consideration, and which, unless $\pi' = \pi$ and $\eloi$
gets stuck in a position of the form $(\dia\be,s)$ with $\dia\be \in H$, 
ends at a position either of the form $(q,s)$ (in which case the match is 
over), or of the form $(\be,s)$ with $q$ not occurring in $\be$.

Similarly a full match $\pi$ of an evaluation game $\EG(\mu 
q.\al,\bbS)@(\mu q.\al,r)$ will have one of the following shapes:
\begin{enumerate}
\item 
$\pi$ is infinite and $\eloi$ looses since this means that $q$ is unfolded
infinitely often;
\item
$\pi$ is finite and has an initial $H$-part $\pi'$ which satisfies 
one of the following:
    \begin{enumerate}
    \item $\pi = \pi'$ and $\eloi$ looses in getting stuck at a diamond formula;
    \item $\pi'$ ends in a position of the form $(\be,s)$ with $q$ not 
    occurring in $\be$; in this case $(\be,s)$ is preceded by a position of the
    form $(\ga,s)$ with $q \sfor \ga \in H$ and $\be$ being either a conjunct 
    or a disjunct of $\ga$.
    \end{enumerate}
\end{enumerate}

\begin{definition}
Let $\phi$ the WMSO-formula $\{ \exists Y_{\be} \mid \be \in H \}.\phi'$,
where $\phi'$ is the conjunction of the following formulas:
\begin{description}
\item[$\mathbf{(\chi_{r})}$] $Y_{\al}(r)$
\item[$\mathbf{(\chi_{\lor})}$] 
   $\bw_{\be\lor\ga \in H}\forall x. (Y_{\be\lor\ga}x \to
      (Y_{\be}x \lor Y_{\ga}x))$
\item[$\mathbf{(\chi_{\land})}$] 
   $\bw_{\be\land\ga \in H}\forall x. (Y_{\be\land\ga}x \to 
      (Y_{\be}x \land Y_{\ga}x))$
\item[$\mathbf{(\chi_{\dia})}$] 
   $\bw_{\dia\be \in H}\forall x. (Y_{\dia\be}x \to 
      \exists y. (Rxy \land Y_{\be}y))$
\item[$\mathbf{(\chi_{\mu})}$] 
   $\forall x. (Y_{q}x \to Y_{\al}x)$
\item[$\mathbf{(\chi_{\ML})}$] 
   $\bw_{q \not\sfor \psi \in H}\forall x. (Y_{\psi}x \to 
      \ST{x}(\psi))$
\end{description}
\end{definition}

\begin{proposition}
Let $\bbT$ be a tree with root $r$. 
Then
\[
\bbT,r \forces \mu q.\al \iff \bbT, r \models \phi.
\]
\end{proposition}

\begin{proof}
\fbox{$\Rightarrow$} 
If $\bbT,r \forces \mu q.\al$ then $\eloi$ has a winning strategy $f$ in the 
game $\EG(\mu q.\al,\bbT)@(\mu q.\al,r)$.
For $\be\in H$, define $Y_{\be}$ to be the set of states $t \in T$ such that 
there is a (partial) match $\pi'$ that (i) is consistent with $f$, and such 
that (ii) every position of $\pi'$ is of the form $(\ga,t)$ with $\ga\in H$,
and (iii) the last position of $\pi'$ is of the form $(\be,t)$.

The two key observations are that since $f$ is a winning strategy, all 
$f$-consistent matches are finite, and that because of the shape of formulas
in $H$, the only player who picks successors during the initial $H$-part of
a match is $\eloi$.
As a consequence of K\"onig's Lemma, each set $Y_{\be}$ is finite.

This means that these sets can interpret the second-order variables 
of the WMSO-formula $\phi$.
The details as to why the collection $\{ Y_{\be} \mid \be \in H \}$ 
satisfies the $\chi$-formulas, will be given later.


\fbox{$\Rightarrow$}
Assume that $\bbT, r \models \phi$.
By a slight abuse of notation we will let $\{ Y_{\be} \mid \be \in H \}$
denote a finite set of finite subsets of $T$ such that $\bbT[Y_{\be} 
\mid \be \in H],r \models \phi'$.
%
In order to show that $\bbT,r \forces \mu q.\al$, let $\eloi$ use the 
following strategy in the game $\EG(\mu q.\al,\bbT)@(\mu q.\al,r)$:
\begin{itemize}
\item
at a position of the form $(\be,t)$ with $q \sfor \be$ and $t \in Y_{\be}$,
distinguish cases:
   \begin{itemize}
   \item if $\be = \be_{0} \lor \be_{0}$, pick $i \in \{ 0,1 \}$ such 
   that $t \in Y_{\be_{i}}$; such an $i$ exists because of 
   ($\chi_{\lor}$);
   \item if $\be = \dia\ga$, pick a $u \in T$ such that $Rtu$ and $u 
   \in Y_{\ga}$; such a $u$ exists because of ($\chi_{\dia}$);
   \end{itemize}
\item
at a position of the form $(\psi,t)$ with $q \not\sfor \psi$, if $\bbT,t 
\forces \psi$ then $\eloi$ uses her canonical strategy;
\item
at all other positions, $\eloi$ moves randomly.
\end{itemize}

%For this strategy we can prove the following claim.

\begin{claim}
For all positions $(\be,t)$ that are consistent with the above strategy,
either $q \sfor \be$ and $t \in Y_{\be}$, or $q \not\sfor \be$ and 
$\bbT,t \forces \be$.
\end{claim}

\begin{pfclaim}
By a straightforward induction on the length of partial matches.
\end{pfclaim}

Consider an arbitrary full match $\pi$ that is consistent with this 
strategy.
It easily follows by the above claim that $\eloi$ will not get stuck
(some details to be supplied).

Suppose for contradiction that $\pi$ is infinite, i.e., the variable $q$
is unfolded infinitely often during $\pi$.
Because $\bbT$ is a tree and $\al$ is guarded in $q$, this means that $\pi$ 
passes through infinitely many \emph{distinct} positions of the form 
$(q,t)$.
Then by the claim the set $Y_{q}$ must be infinite, which contradicts the
fact that $Y_{q}$ interprets a WMSO-variable.

It follows that $\pi$ is finite. 
Then by the earlier classification of matches, $\pi$ has an initial 
$H$-part $\pi'$ which ends 
in a position of the form $(\psi,s)$ with $q$ not occurring in $\psi$.
By the above claim, this means that $\bbT,t \forces \psi$, and so $\eloi$'s
canonical strategy, which she uses in the remainder of the match, guarantees
that she wins the match.

In other words, we have provided $\eloi$ with a winning strategy in the 
game $\EG(\mu q.\al,\bbT)@(\mu q.\al,r)$, as required.
\end{proof}

